Automated NRQCD and NRQED simulations of quarkonium and leptonium production with P-wave states and physical-mass effects

We present the $\texttt{MadSONS}$ module, which extends the $\texttt{MadGraph5_aMC@NLO}$ framework by providing a fully automated solution for the simulation of arbitrary tree-level production processes involving non-relativistic bound states. More specifically, we focus on the production of quarkonia and leptonia in non-relativistic QCD and QED, respectively. This work constitutes the next step in the programme initiated in arXiv:2510.26773, where the colour and spin projectors required for S-wave states were first incorporated into $\texttt{MadGraph5_aMC@NLO}$. In the present development, we implement the remaining projectors associated with orbital and total angular momentum, thereby enabling the event generation of processes involving P-wave states. The derivatives required for the orbital-angular-momentum projection are evaluated using dual numbers. In addition, we implement a momentum-reshuffling procedure that accounts for physical bound-state mass effects in the phase space. The resulting framework applies to a wide range of collider environments while remaining compatible with standard multi-purpose Monte Carlo event generators for parton showering and hadronisation. As a first phenomenological application, we revisit $J/\psi + \psi(2{\rm S})$ production at the LHC and obtain an improved description of the LHCb data.

==> feynman/lep_3.tex <==
% Created with FeynGame
% Include with input{lep_3.tex}
% Width can be set with \def\svgwidth{...} and a scaling with \def\svgscale{...}
% These options have to be set before the import statement and only apply to one included file
\begingroup%
  \makeatletter%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{595.32000732bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \parbox[c][][c]{\unitlength}{%
    \begin{picture}(1,0.6361185983827493)%
      \put(0,0){\includegraphics[width=\unitlength,viewport = 0 0 213 135]{feynman/lep_3.eps}}%
      \put(0.0830188665107254,0.5703504050195699){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$e^-$}}}}}}%
      \put(0.08301887357973989,0.06145553126168058){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$e^+$}}}}}}%
      \put(0.8776280436554367,0.564420488002808){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$\gamma$}}}}}}%
      \put(0.4743935309973046,0.2641509433962264){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$\gamma^\ast$}}}}}}%
      \put(0.6820062666195713,0.3152610422744459){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$\ell^-$}}}}}}%
      \put(0.6814546094676578,0.07719493322102994){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$\ell^+$}}}}}}%
      \put(0.9180512129380054,0.1967654986522911){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$\chi_{\ell J}$}}}}}}%
    \end{picture}%
  }%
\endgroup%

